On Well-posed Boundary Conditions for the Linear Non-homogeneous Moment Equations in Half-space

We propose a necessary and sufficient condition for the well-posedness of the linear non-homogeneous Grad moment equations in half-space. The Grad moment system is based on Hermite expansion and regarded as an efficient reduction model of the Boltzmann equation. At a solid wall, the moment equations are commonly equipped with a Maxwell-type boundary condition named the Grad boundary condition. We point out that the Grad boundary condition is unstable for the non-homogeneous half-space problem. Thanks to the proposed criteria, we verify the well-posedness of a class of modified boundary conditions. The technique to make sure the existence and uniqueness mainly includes a well-designed preliminary simultaneous transformation of the coefficient matrices and Kreiss' procedure about the linear boundary value problem with characteristic boundaries. The stability is established by a weighted estimate. At the same time, we obtain the analytical expressions of the solution, which may help solve the half-space problem efficiently.

==> num.tex <==
\section{Numerical Verifications}
The realistic applications of the linear non-homogeneous half-space
problems can be found in the textbook \cite{Sone2007}. To avoid 
introducing more backgrounds, we only solve a toy model numerically
to support our theory.

We consider the Couette flow with the BGK collision term. Assume
the moment order $M\geq 3$ is an odd number. Then we write 
$W_e=(f_1,f_3,...,f_M)^T$ and $W_o=(f_2,f_4,...,f_{M-1})^T$,
and the moment system in half-space reads as
\[
	\begin{bmatrix} \+0 & \+M \\ \+M^T & \+0 \end{bmatrix}
	\od{}{y}\begin{bmatrix} W_e \\ W_o \end{bmatrix}
	= -\begin{bmatrix} 0 & \\ & \+I_{M-1}\end{bmatrix} 
	\begin{bmatrix} W_e \\ W_o \end{bmatrix} + h.
\]
Here $\+I_{M-1}$ is the $(M-1)$-th order identity matrix and
$\+M$ is a lower triangular matrix with
\[
	\+M = \begin{bmatrix} 1 &  & &\\
		 		\sqrt{2} & \sqrt{3} & &\\
		  &  \ddots & \ddots & \\	 
		 && \sqrt{M-3} & \sqrt{M-2} \\
			 & & & \sqrt{M-1} 
	\end{bmatrix}\in\bbR^{m\times n},
\]
where $m+n=M,\ m=n+1.$ The non-homogeneous term is

太麻烦了, 不算了.

